3D Registration for Self-Occluded Objects in Context

While much progress has been made on the task of 3D point cloud registration, there still exists no learning-based method able to estimate the 6D pose of an object observed by a 2.5D sensor in a scene. The challenges of this scenario include the fact that most measurements are outliers depicting the object's surrounding context, and the mismatch between the complete 3D object model and its self-occluded observations. We introduce the first deep learning framework capable of effectively handling this scenario. Our method consists of an instance segmentation module followed by a pose estimation one. It allows us to perform 3D registration in a one-shot manner, without requiring an expensive iterative procedure. We further develop an on-the-fly rendering-based training strategy that is both time- and memory-efficient. Our experiments evidence the superiority of our approach over the state-of-the-art traditional and learning-based 3D registration methods.

==> table/inference_time_h.tex <==
\begin{table*}[b]
    \centering
    % \setlength{\abovecaptionskip}{.3cm}
    % \setlength{\belowcaptionskip}{-5pt}
    \setlength{\tabcolsep}{6.5mm}{
    \begin{tabular}{@{}lcccccc@{}}
    \toprule
    \textbf{Points}      & \textbf{ICP} & \textbf{FGR} & \textbf{TEASER++} & \textbf{DCP} & \textbf{PRNet} & \textbf{Ours-OT} \\ \midrule
    \textbf{512}         & 0.018        & 0.032        & 0.025        & 0.013        & 0.051          & 0.033         \\
    \textbf{1024}        & 0.028        & 0.059        & 0.085        & 0.018        & 0.075          & 0.052         \\
    \textbf{2048}        & 0.054        & 0.132        & 0.249        & 0.053        & 0.141          & 0.112         \\ \bottomrule
    \end{tabular}}
    \caption{\label{tab:inference_time} Inference time (in seconds).}
\end{table*}

==> tex/supplymentary.tex <==
\section{Supplymentary}

In \Cref{tudl_1,tudl_2,tudl_3}, we provide additional qualitative results on the three test sequences of the TUD-L dataset~\cite{Hodan18}.
Furthermore, we provide qualitative results for every class in ModelNet40~\cite{Wu15,Sedaghat16} in \Cref{blenderproc_1,blenderproc_2,blenderproc_3,blenderproc_4,blenderproc_5,blenderproc_6,blenderproc_7,blenderproc_8}.

% \input{fig/supply_figs/tudl_1}
% \input{fig/supply_figs/tudl_2}
% \input{fig/supply_figs/tudl_3}
% \input{fig/supply_figs/blenderproc_1}
% \input{fig/supply_figs/blenderproc_2}
% \input{fig/supply_figs/blenderproc_3}
% \input{fig/supply_figs/blenderproc_4}
% \input{fig/supply_figs/blenderproc_5}
% \input{fig/supply_figs/blenderproc_6}
% \input{fig/supply_figs/blenderproc_7}
% \input{fig/supply_figs/blenderproc_8}

\clearpage
\clearpage
\clearpage
\clearpage
\clearpage
\clearpage
